Remarks on multi-dimensional noncommutative generalized Brownian motions

We consider certain questions pertaining to noncommutative generalized Brownian motions with multiple processes. We establish a framework for generalized Brownian motion with multiple processes similar to that defined by Guta and prove multi-dimensional analogs of some results of Guta and Maassen. We then consider examples of processes indexed by a two-element set and characterize the function on I-indexed pair partitions associated via the I-indexed generalized Brownian motion construction to certain pairs of representations connected to certain spherical representations of infinite symmetric groups. In doing so, we generalize the notion (introduced by Bozejko and Guta) of the cycle decomposition of a pair partition. We then generalize Guta's q-product of generalized Brownian motions to a product corresponding to a (possibly infinite) matrix $(q_{ij})$ and show that this $q_{ij}$-product satisfies a central limit theorem.

==> thesis-intro.tex <==
\secondarydivision{Brownian motions}
The study of classical Brownian motion has its origins in the world of physics.
Einstein introduced the concept to explain the random motion of small particles suspended in a fluid, naming the phenomenon after the botanist Robert Brown, who had observed the motion of grains of pollen in water under a microscope.

The probabilistic model of a one-dimensional Brownian motion, sometimes called a Wiener process, is a real-valued stochastic process $B_t$ having the following properties:
\begin{enumerate}
\item If $t_0<t_1<\ldots< t_n$ then the increments $B(t_0)$, $B(t_1)-B(t_0)$,\ldots, $B(t_n)-B(t_{n-1})$ are independent.
\item If $s,t\ge 0$ then $B(s+t)-B(s)$ is a centered Gaussian random variable with variance $t$.
\item The map $t\mapsto B_t$ is continuous with probability $1$.
\end{enumerate}
There is also a notion of multidimensional Brownian motion with independent processes $(B^j(t))_{j\in\IndexSet}$ indexed by a set $\IndexSet$, with each individual process being a (one-dimensional) Brownian motion.

Over the years, a number of realizations of classical Brownian motion have been developed.
One construction, credited to L\'evy \cite{Levy} and Ciesielski \cite{Ciesielski59} uses random series with respect to an orthonormal basis in $L^2([0,1])$ to construct a Brownian motion on $[0,1]$.
Another construction uses an invariance theorem of Donsker \cite{Donsker} to construct Brownian motion as a limit of linearly interpolated random walks.
A detailed treatment of classical Brownian motion, including these and several additional constructions, can be found in \cite{SP}.
\secondarydivision{Noncommutative probability theory}
Noncommutative probability theory (c.f. \cite{VDN}) is an analog of classical probability theory in which multiplication of random variables is not necessarily commutative.
A noncommutative probability space is a pair $(\ncps,\varphi)$ where $\ncps$ is a $*$-algebra and $\varphi:\ncps\to\BC$ is a positive unital linear functional.
The elements $a\in\ncps$ are called random variables, and the linear functional $\varphi$ takes the place of the expectation functional of classical probability theory.

Given a noncommutative probability space $(\ncps,\phi)$, for elements $X_1,\ldots, X_n\in\ncps$ the distribution $\mu$ of a finite family $(f_\iota)_{\iota\in I}$ is the linear functional on $\BC\left<X_\iota, X_\iota^*|\iota\right>$, the algebra of noncommutative polynomials in the variables $\{X_\iota, X_\iota^*| \iota\in I\}$, defined by $\mu(P) = \phi(h(P))$.
Here $h:\BC\left<X_\iota, X_\iota^*|\iota\right>\to\ncps$ is the unique algebra homomorphism such that $h(X_\iota)=f_\iota$ and $h(X_\iota^*)=f_\iota^*$.
The values of $\mu$ on monomials are called the moments of the family.

It is common to study noncommutative probability with some additional assumptions on the algebra $\ncps$ and the functional $\varphi$.
For instance, $\ncps$ may be assumed to be a von Neumann algebra, and $\varphi$ weakly continuous, in which case the pair $(\ncps,\varphi)$ is called a $W^*$ probability space.
The following example establishes classical probability spaces as a special case of noncommutative probability spaces.
\begin{example}\label{ex:ncps}
Suppose that $(\Omega, \mathcal F, P)$ is a classical probability space, i.e. $\Omega$ is a set, $\mathcal F$ is a $\sigma$-field ($\sigma$-algebra) on $\Omega$, and $P$ is a measure on the space $(\Omega,\mathcal F)$ such that $P(\Omega)=1$. 
Then $L^\infty(\Omega, P)$ is a von Neumann algebra acting on the Hilbert space $L^2(\Omega, P)$ by pointwise multiplication.
Letting $E$ denote expected value with respect to $P$, the pair $(L^\infty(\Omega), E)$ is a $W^*$-probability space.
Moreover, the classical moments of a family $(f_\iota)_{\iota\in I}$ of bounded random variables are the same as the moments in the noncommutative sense just described.
\end{example}
As should be clear from the example, we do not disallow the possibility that a noncommutative probability space be commutative.
That is, we use the word ``noncommutative'' to mean ``not necessarily commutative.''

The most important noncommutative probability theory is free probability, which was initiated by Voiculescu in the 1980s.
Free probability is the study of noncommutative probability theory with a notion of independence based on the free product.
Many important notions of classical probability theory, ranging from the central limit theorem to entropy find counterparts in classical probability theory. 
We refer the reader to the book \cite{VDN} for an excellent introduction to free probability theory.   
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\secondarydivision{Noncommutative generalized Brownian motions}
Hudson and Parthasarathy in \cite{HP} constructed a ``Boson quantum Brownian motion,'' an operator-valued process whose moments coincided with those of classical Brownian motion.
The coincidence of moments ensures the existence of a unitary equivalence between the operator-valued process and the classical processes acting by pointwise multiplication on a suitable $L^2$ space.

The operator-valued processes of Hudson and Parthasarathy act on the Bosonic Fock space of the complex Hilbert space $L^2(\BR^+,\BC)$.
The Boson quantum Brownian motion arises as a sum of creation and annihilation operators associated to $\chi_{[0, t]}$ on the Bosonic Fock space.
That is, if the creation and annihilation operators associated to $f\in L^2(\BR^+,\BC)$ on the Bosonic Fock space are denoted by $a^*(f)$ and $a(f)$, respectively, then the Boson quantum Brownian motion is given by $t\mapsto a^*(\chi_{[0, t]})+a(\chi_{[0, t]})$.

The independence of increments in the operator-valued processes can be seen as a consequence of the orthogonality of the characteristic functions on disjoint intervals.
However, the definition of continuity with probability 1 makes explicit reference to the underlying probability space, so it is not entirely clear how to translate this axiom to the operator setting.
One effort to define a notion of continuity for operator processes can be found in \cite{Luczak}, but we will not make use of it here.

The Hudson-Parthasarathy Boson quantum Brownian motion finds a natural analog in the setting of free probability, with the full Fock space replacing the Bosonic Fock space.
Voiculescu showed in \cite{V1985} that the sum of creation and annihilation operators on the full Fock space are distributed according to the Wigner semicircle law, which is the free analog of the classical Gaussian distribution.
Considering the sum of full Fock space creation and annihilation operators associated to the characteristic function $\chi_{[0, t]}$ gives a free analog of classical Brownian motion.

Bo{\.z}ejko and Speicher initiated the study of noncommutative generalized Brownian motions, introducing operators satisfying an interpolation between Fermionic and Bosonic commutation relations \cite{BS1991}.
Specifically, for $q\in [-1,1]$ and a complex Hilbert space $\HH$, they constructed a $q$-deformed Fock space $\FS_q(\HH)$ with creation operators
$c^*(f)$ and annihilation operators $c(f)$ for $f\in\HH$ satisfying the relations
\begin{equation}
 c(f)c^*(g)-qc^*(g)c(f)=\left<f,g\right>\cdot 1.
\end{equation}
The case $q=0$ gives the creation and annihilation operators on the full Fock space and the case $q=1$ gives creation and annihilation operators on the Bosonic Fock space.
Consequently, one can view the sum of creation and annihilation operators on the $q$-Fock space as a generalization of the classical and free Brownian motions.
These $q$-Brownian motions were investigated in detail in \cite{BKS}.


Subsequently, Bo{\.z}ejko and Speicher  in \cite{BS1996} developed a broader framework of generalized Brownian motion which incorporated their $q$-Brownian motion.
In this setting, one considers the algebra obtained by applying the Gelfand-Naimark-Segal construction (c.f. \cite[Theorem I.9.6]{Davidson}) to the  free tensor algebra of a real Hilbert space $\HH$ with certain states, called Gaussian states, associated to a class of functions, called positive definite, on pair partitions via a so-called pairing prescription.

{Gu{\c{t}}{\u{a}} and Maassen further explored this notion of generalized Brownian motion \cite{GM1,GM2}.
They showed that Gaussian states $\rho_\Pt$ can be instead characterized by sequences of complex Hilbert spaces $(V_n)_{n=1}^\infty$ with densely defined maps $j_n:V_n\to V_{n+1}$ and representations $U_n$ of the symmetric group $S_n$ on $V_n$ satisfying an intertwining relation, data which give rise to a symmetric Fock space with creation and annihilation operators.
They also provided an algebraic characterization of the notion of positive definiteness for a function $\Pt$ on pair partitions.
Separately in \cite{GM2}, they examined a class of Brownian motions arising from the combinatorial notion of species of structure.

Bo{\.z}ejko and {Gu{\c{t}}{\u{a}} \cite{BG} considered a special case of the  generalized Brownian motion of {Gu{\c{t}}{\u{a}} and Maassen arising from $II_1$-factor representations of the infinite symmetric group $S_\infty$ constructed by Vershik and Kerov \cite{VK}.
Lehner \cite{Lehner} considered  these  generalized Brownian motions in the context of exchangeability systems, which generalize various notions of independence and give rise to cumulants analogous to the well-known free and classical cumulants.
Recent work of Avsec and Junge \cite{AJ} offers another point of view on the subject of noncommutative Brownian motion.


In \cite{Guta} {Gu{\c{t}}{\u{a}} extended the notion of generalized Brownian motion to multiple processes indexed by some set $\IndexSet$.
He went on to define for $-1\le q\le 1$  a $q$-product of generalized Brownian motions interpolating between the graded tensor product previously considered by Mingo and Nica \cite{MN} ($q=-1$), the reduced free product \cite{V1985} ($q=0$) and the usual tensor product ($q=1$).
He also showed that this $q$-product obeys a central limit theorem as the size of the index set $\IndexSet$ grows.

In this thesis, we explore certain additional questions pertaining to the $\IndexSet$-indexed generalized Brownian motions.
We will begin by establishing the basic notions, and, as a warmup, considering a simple case of a generalized Brownian motion arising from a tensor product of representations of the infinite symmetric group $S_\infty$.
We compute the functions on pair partitions associated to the Gaussian states in this context.
We then proceed to consider the generalized Brownian motions associated to spherical representations of the Gelfand pair $(S_\infty\times S_\infty,S_\infty)$.
Here again we give a combinatorial formula for the function on pair partitions arising from the associated Gaussian states.
In the course of doing so we generalize the notion, introduced by Bo{\.z}ejko and {Gu{\c{t}}{\u{a}} \cite{BG}, of a cycle decomposition of a pair partition to pair partitions with two colors. 
We then specialize to a specific case related to a countable family of spherical representations of the Gelfand pair $(S_\infty\times S_\infty,S_\infty)$ which gives bounded operators.
We conclude by generalizing {Gu{\c{t}}{\u{a}}'s $q$-product of generalized Brownian motions to a $q_{ij}$ product, where $i,j\in\IndexSet$ and showing that a central limit theorem holds when $q_{ij}=q_{ji}$ and the $q_{ij}$ are periodic in both $i$ and $j$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
